Permutation-Invariant Relational Network for Multi-person 3D Pose Estimation

The recovery of multi-person 3D poses from a single RGB image is a severely ill-conditioned problem due to the inherent 2D-3D depth ambiguity, inter-person occlusions, and body truncations. To tackle these issues, recent works have shown promising results by simultaneously reasoning for different people. However, in most cases this is done by only considering pairwise person interactions, hindering thus a holistic scene representation able to capture long-range interactions. This is addressed by approaches that jointly process all people in the scene, although they require defining one of the individuals as a reference and a pre-defined person ordering, being sensitive to this choice. In this paper, we overcome both these limitations, and we propose an approach for multi-person 3D pose estimation that captures long-range interactions independently of the input order. For this purpose, we build a residual-like permutation-invariant network that successfully refines potentially corrupted initial 3D poses estimated by an off-the-shelf detector. The residual function is learned via Set Transformer blocks, that model the interactions among all initial poses, no matter their ordering or number. A thorough evaluation demonstrates that our approach is able to boost the performance of the initially estimated 3D poses by large margins, achieving state-of-the-art results on standardized benchmarks. Additionally, the proposed module works in a computationally efficient manner and can be potentially used as a drop-in complement for any 3D pose detector in multi-people scenes.

==> fig_05_qual_nba.tex <==
\begin{figure*}[t!]
% \begin{figure}[H]
  \vspace{-0.1cm}
  \centering
  \includegraphics[width=0.8\linewidth, trim={0.1cm 0.1cm 0cm 0}, clip = true]{figures/NBA.png}

  \vspace{-0.4cm}
  \caption{\small{\textbf{Qualitative results.} On NBA2K~\cite{zhu_2020_eccv_nba} and COCO~\cite{coco} datasets. In each case we plot the ground truth, and the estimated 3D poses, overlayed with the initialization. Additional examples are provided in the supplemental material.
  }}
  \label{fig:qualitative_nba}
  \vspace{-0.3cm}
\end{figure*}


==> fig_06_qual_coco.tex <==
\begin{figure*}[t!]
  \vspace{0.1cm}
  \includegraphics[width=\linewidth, trim={0.1cm 0.1cm 0cm 0}, clip = true]{figures/coco.png}
  \vspace{0.1cm}
  \caption{\small{\textbf{Qualitative results.} On COCO. In each case we plot the ground truth, and the estimated 3D poses, overlayed with the initialization. Additional examples are provided in the supplemental material.
  }}
  \label{fig:qualitative_coco}
  \vspace{-0.4cm}
\end{figure*}


==> tables/table_NBA_PCK.tex <==
\begin{table}[]
\centering
\caption{Qualitative comparison for NBA dataset with 3DPCK\textsubscript{rel} metric.}
\label{tab:nba_pck}

\begin{tabular}{l|lllll}
\hline
\multicolumn{1}{c|}{Method} & \multicolumn{5}{c}{All people  $\uparrow$}                          \\ \hline
              & Cory & Glen & Oscan & \multicolumn{1}{l|}{Toman} & Avg  \\
RootNet             & 62.6 & 63.0 & 69.7  & \multicolumn{1}{l|}{65.1}  & 65.1 \\
Pi-Net (re-trained) & 68.3 & 66.5 & 71.9  & \multicolumn{1}{l|}{67.7}  & 68.6 \\ \hline
\textbf{Ours} & \textbf{71.3} & \textbf{67.7} & \textbf{74.7} & \multicolumn{1}{l|}{\textbf{71.2}} & \textbf{71.2} \\ \hline
\end{tabular}
\vspace{0.2cm}
\end{table}

==> tables/table_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\caption{Ablation Results. See text for details.}
\label{tab:ablation}
  \resizebox{1.0 \textwidth}{!}{%
\begin{tabular}{l|l|ccc|cc}
\hline
                              &                                    & \multicolumn{3}{c|}{All people} &               &               \\ \cline{2-7} 
                       & \multicolumn{1}{c|}{Metric}        & PCK\textsubscript{rel}$\uparrow$ & PCK\textsubscript{abs}$\uparrow$ & AUC\textsubscript{rel}$\uparrow$       & MPJPE$\downarrow$ & MPJPE-PA$\downarrow$ \\ \hline
\multirow{4}{*}{MuPoTS-3D}    & Initial (RootNet)                  & 81.2      & 31.4     & 39.5     & 134.9         & 93.3          \\
                              & Baseline – no interaction          & 79.9      & 35.4     & 40.3     & 136.4         & 95.1          \\
                              & Baseline – scene interaction       & 80.3      & 40.6     & 40.1     & 134.5         & 96.1          \\
                       & \textbf{Ours – people interaction} & \textbf{85.8} & \textbf{44.1} & \textbf{46.1} & \textbf{104.8} & \textbf{79.7}     \\ \hline
\multirow{4}{*}{NBA2K} & Initial (RootNet)                  & 65.1          & -  & 34.8          & 154.1          & 119.7             \\
                              & Baseline – no interaction          & 62.8      & -      & 32.6     & 169.5         & 137.6         \\
                              & Baseline – scene interaction       & 22.7      & -      & 16.7     & 892.7         & 535.9         \\
                       & \textbf{Ours – people interaction} & \textbf{71.2} & -           & \textbf{36.4} & \textbf{131.9} & \textbf{102.7}    \\ \hline
\multirow{4}{*}{CMU Panoptic} & Initial (RootNet)                  & -         & -        & -        & 158.1         & 124.1         \\
                              & Baseline – no interaction          & -         & -        & -        & 156.1         & 122.3         \\
                              & Baseline – scene interaction       & -         & -        & -        & 293.7         & 154.1         \\
                              & \textbf{Ours – people interaction} & -         & -        & -        & \textbf{85.6} & \textbf{66.0} \\ \hline
\end{tabular}}
\end{table}

==> tables/table_ablation_2.tex <==
% \usepackage{multirow}


\begin{table}
\centering
\caption{Ablation Results. See text for details.}
\label{tab:ablation}
\begin{tabular}{c||l||c||c}
\multicolumn{1}{l||}{}     & \multicolumn{1}{c||}{Metric}       & MPJPE [mm]$\downarrow$     & MPJPE-PA [mm]$\downarrow$  \\ 
\hline\hline
\multirow{4}{*}{MuPoTS-3D} & Initial (RootNet)                  & 134.9          & 93.3           \\ 
\cline{2-4}
                           & Baseline – no interaction          & 136.4          & 95.1           \\ 
\cline{2-4}
                           & Baseline – scene interaction       & 134.5          & 96.1           \\ 
\cline{2-4}
                           & \textbf{Ours – people interaction} & \textbf{104.8} & \textbf{79.7}  \\ 
\hline\hline
\multirow{4}{*}{Panoptic}  & Initial (RootNet)                  & 158.1          & 124.1          \\ 
\cline{2-4}
                           & Baseline – no interaction          & 156.1          & 122.3          \\ 
\cline{2-4}
                           & Baseline – scene interaction       & 293.7          & 154.1          \\ 
\cline{2-4}
                           & \textbf{Ours – people interaction} & \textbf{85.6}  & \textbf{66.0} 
\end{tabular}
\end{table}

==> tables/table_mupots_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Quantitative comparison with state-of-the-art methods on the MuPoTS-3D dataset.
*Results shown for these methods are merely referential as they are not re-trained with the same data as ours. They are trained with various datasets, in most cases, and more data than our model.}
\label{tab:mupots}
  \resizebox{1.0 \textwidth}{!}{%
\begin{tabular}{l|ccc|ccc|lll}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
  \multicolumn{3}{c|}{All people} &
  \multicolumn{3}{c|}{Matched people} &
  \multicolumn{3}{c}{\multirow{2}{*}{Datasets training}} \\ \cline{2-7}
\multicolumn{1}{c|}{} & PCK\textsubscript{rel}$\uparrow$   & PCK\textsubscript{abs}$\uparrow$  & AUC\textsubscript{rel}$\uparrow$  & PCK\textsubscript{rel}$\uparrow$ & PCK\textsubscript{abs}$\uparrow$  & AUC\textsubscript{rel}$\uparrow$  & \multicolumn{3}{c}{}                        \\ \hline
Initial (RootNet~\cite{Moon_2019_ICCV_3DMPPE})     & 81.2 & 31.4    & 39.5    & 82.5 & 32.0    & 40.2    & \multicolumn{3}{l}{MuCo + COCO}             \\
PI-Net~\cite{guo2021pi}         & 82.5 & -       & -       & 83.9 & -       & -       & \multicolumn{3}{l}{MuCo}                    \\
PI-Net (fine-tunned)  & 82.8 & -       & 43.9    & 84.3 & -       & 44.79   & \multicolumn{3}{l}{MuPots Cross Validation} \\
\textbf{Ours} &
  \textbf{85.8} &
  \textbf{44.1} &
  \textbf{46.13} &
  \textbf{87.3} &
  \textbf{45.0} &
  \textbf{46.91} &
  \multicolumn{3}{l}{MuPots Cross Validation} \\ \hline
HMOR*                 & 82   & 43.8    & 43.5    & -    & -       & -       & \multicolumn{3}{l}{MuCo + COCO +}           \\
HDNet*                & -    & -       & -       & 83.7 & 35.2    & -       & \multicolumn{3}{l}{MuCo}                    \\
SMAP*                 & 73.5 & 35.4    & -       & 80.5 & 38.7    & 42.7    & \multicolumn{3}{l}{MuCo + COCO}             \\ \hline
\end{tabular}}
\vspace{0.2cm}
\end{table}


==> tables/table_panoptic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Quantitative comparison in the CMU Panoptic dataset. *RootNet model was fine-tuned with CMU Panoptic data for us to have a better initialization. Ours(1) uses initialization from RootNet model using original network parameters. Ours(2) uses initialization from RootNet with fine-tuned weights. }
\label{tab:panoptic}
  \resizebox{1.0 \textwidth}{!}{%
\begin{tabular}{c|l|cccccc|cccccc}
\hline
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
  \multicolumn{6}{c|}{MPJPE {[}mm.{]} $\downarrow$} &
  \multicolumn{6}{c}{MPJPE – PA {[}mm.{]} $\downarrow$} \\ \cline{3-14} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{} &
  Haggling &
  Mafia &
  Ultim. &
  Pizza &
  Avg All &
  Avg Seq. &
  Haggling &
  Mafia &
  Ultim. &
  Pizza &
  Avg All &
  Avg Seq. \\ \cline{1-2}
\multirow{4}{*}{Refinement} &
  RootNet &
  116.8 &
  149.7 &
  168.1 &
  186.5 &
  158.1 &
  - &
  97.6 &
  117.2 &
  130.2 &
  144.2 &
  124.1 &
  - \\
 &
  \textbf{Ours (1)} &
  75.2 &
  77.3 &
  84.1 &
  101.9 &
  85.6 &
  - &
  59.9 &
  61.9 &
  66.7 &
  74.0 &
  66.0 &
  - \\
 &
  RootNet* &
  83.3 &
  107.9 &
  106.0 &
  118.4 &
  106.7 &
  103.9 &
  74.6 &
  94.2 &
  93.3 &
  101.8 &
  93.1 &
  91.0 \\
 &
  \textbf{Ours (2)} &
  \textbf{59.4} &
  \textbf{68.9} &
  \textbf{67.2} &
  \textbf{86.4} &
  \textbf{72.5} &
  \textbf{70.5} &
  \textbf{48.8} &
  \textbf{55.7} &
  \textbf{52.7} &
  \textbf{66.4} &
  \textbf{57.4} &
  \textbf{55.9} \\ \hline
\multirow{3}{*}{End-to-End} &
  Zanfir et al.~\cite{zanfir_multipeople_nips18} &
  72.4 &
  78.8 &
  66.8 &
  94.3 &
  - &
  78.1 &
  - &
  - &
  - &
  - &
  - &
  - \\
 &
  SMAP~\cite{smap_eccv2020} &
  63.1 &
  60.3 &
  56.6 &
  \textbf{67.1} &
  - &
  61.8 &
  - &
  - &
  - &
  - &
  - &
  - \\
 &
  HMOR~\cite{HMOR2020} &
  \textbf{50.9} &
  \textbf{50.5} &
  \textbf{50.7} &
  68.2 &
  \textbf{51.6} &
  - &
  - &
  - &
  - &
  - &
  - &
  - \\ \hline
\end{tabular}}
  \vspace{-0.1cm}
\end{table}

==> tables/table_running_time.tex <==
\begin{table}
\centering
\caption{Running time, memory and computation complexity comparison. The \ti{Data} column refers to the approximate magnitude of amount of data used to train the model.}
\label{tab:running_time}
  \resizebox{0.4\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
Method & \multicolumn{1}{l}{\# Params} & \multicolumn{1}{l}{FLOPS} & \multicolumn{1}{l}{Training Data} & \multicolumn{1}{l}{Time (ms)} \\ \midrule
RootNet~\cite{Moon_2019_ICCV_3DMPPE}       & 167.7M         & 547.8G        & 100K         & 250.7      \\
HMOR~\cite{HMOR2020}            & 45.0M          & 320.2G        & 100K         & -          \\
SMAP~\cite{smap_eccv2020}            & 1379M          & -             & 100K         & 57         \\ \midrule
Ours & 0.09M & 5.1M & 10K & 2 \\ \bottomrule
\end{tabular}}
  \vspace{-0.1cm}
\end{table}
